Variable Metric Proximal Gradient Method with Diagonal Barzilai-Borwein Stepsize

Variable metric proximal gradient (VM-PG) is a widely used class of convex optimization method. Lately, there has been a lot of research on the theoretical guarantees of VM-PG with different metric selections. However, most such metric selections are dependent on (an expensive) Hessian, or limited to scalar stepsizes like the Barzilai-Borwein (BB) stepsize with lots of safeguarding. Instead, in this paper we propose an adaptive metric selection strategy called the diagonal Barzilai-Borwein (BB) stepsize. The proposed diagonal selection better captures the local geometry of the problem while keeping per-step computation cost similar to the scalar BB stepsize i.e. $O(n)$. Under this metric selection for VM-PG, the theoretical convergence is analyzed. Our empirical studies illustrate the improved convergence results under the proposed diagonal BB stepsize, specifically for ill-conditioned machine learning problems for both synthetic and real-world datasets.

==> 030consensus.tex <==
% !TEX root = icml_vmpg.tex

% consensus
\begin{figure*}[!h]
\centering
%
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{FIG/fig_cons_LS_small.png}
  \caption{Constrained LS ($N=2500$)}
  \label{fig:sub31}
\end{subfigure} ~%
% \caption{(a) ROC curves on synthetic data yield similar results to VS-MRF (but with greatly improved scalability)}
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{FIG/fig_cons_LS_large.png}
  \caption{Constrained LS ($N=20000$)}
  \label{fig:sub32}
\end{subfigure}~%
% \caption{(a) ROC curves on synthetic data yield similar results to VS-MRF (but with greatly improved scalability)}
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{FIG/fig_cons_LR_small.png}
  \caption{Constrained LR ($N=2500$)}
  \label{fig:sub33}
\end{subfigure}~
\begin{subfigure}[t]{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{FIG/fig_cons_LR_large.png}
  \caption{Constrained LR ($N=10000$)}
  \label{fig:sub34}
\end{subfigure}\\

\vspace{0mm}
\caption{Typical convergence behaviour for PG (BB), VM-PG(local BB), and VM-PG(local DBB) for consensus problems using different sample sizes for synthetic data with the same node number and dimension ($N_{node},n$)$=$($10,100$)}
\vspace{-5pt}
\label{fig:consensus}
\end{figure*}


Finally, we extend the notion of diagonal metric for consensus optimization. Consensus optimization is a widely used framework for solving large-scale machine learning problems in a distributed setting \cite{boyd2011distributed,zhang2012efficient,dhar2015admm}. A typical formulation follows
\begin{align}
\minimize{x_1,\ldots, x_{N_{\mathrm{node}}}\in \reals^n} \sum_{j=1}^{N_{\mathrm{node}}} f_j(x_j) + \delta_{\mathcal{C}}(x_1, \ldots, x_{N_{\mathrm{node}}}). \label{prob:consensus}
\end{align}
where $N_{node}$ is the number of distributed nodes. For each node $j \in \{1 \ldots N_{node}\}$, $f_j : \reals^n \rightarrow \reals$ are convex and differentiable functions with the data $\mathcal{D}_j$. Here, $x_j \in \reals^n$ are the local copies of the shared variable constrained by the consensus set, $\mathcal{C} = \{(x_1\ldots,x_{N_{\mathrm{node}}}\mid x_1= \cdots=x_{N_{\mathrm{node}}}\}$. $\delta_\mathcal{C}$ is the indicator function on $\mathcal{C}$. 
% \xhdr{Remark} Such a separate weighted update can takes into consideration the distribution of data and variability in information at different nodes. For example, for traditional classification and regression problems where the local loss function is proportional to the data subset size at a particular node \cite{zhang2012efficient,dhar2015admm}; the node with the larger data size is likely to provide more information. Hence, the update from such a node should be weighed more in the consensus step. In the following metric slection, this will be possible in the current framework through the weighted updates. Further, this framework is also desirable for advanced machine learning problems with different loss functions over several nodes. This is seen in problems like,  robust estimation \cite{suykens2002weighted}, multi-task learning \cite{xu2014multi} etc. 

% Now we introduce the extended diagonal metric selections for consensus optimization. 


\subsection{5.1 Metric selections for consensus optimization}
% \subsubsection{Global BB-type stepsize} Equation \eqref{prob:consensus} can be represented in its canonical form \eqref{cvxopt_composition} as:- $f(x) = \sum_{j=1}^{N_{\mathrm{node}}} f_j(x_j)$ and $g(x)=\delta_{\mathcal{C}}(x_1, \ldots, x_{N_{\mathrm{node}}})$ for $x = \{x_1,\ldots, x_{N_{\mathrm{node}}}\} \in \reals^{{N_{\mathrm{node}}}n}$. Following Section \ref{sec:metric}, the \textit{scalar} \eqref{eq:bb_hybrid} and \textit{diagonal} \eqref{eq:dbb_solution} BB stepsizes can be computed by referring to global information, i.e., $\{x_j,f_j(x_j) \}_{j=1}^{N_{\mathrm{node}}}$. Thus, for the rest of this section we will refer to these as $\alpha_{\text{global BB}}^k(s^k, y^k)$ and $U_{\text{global DBB}}^k(s^k, y^k)$ respectively. %\youngsuk{one line more}
%However, for both these cases, computing \eqref{eq:bb12} requires global information, i.e., $\{x_j,f_j(x_j) \}_{j=1}^M$. For the rest of this section we will refer to these two approaches in \eqref{eq:bb_hybrid} and \eqref{eq:dbb_solution} as $\alpha_{\text{global BB}}^k(s^k, y^k)$ and $U_{\text{global DBB}}^k(s^k, y^k)$ respectively. However, for consensus problems computing such global stepsizes can be disadvantageous, due to the communication overhead between several agents (nodes). 
% \subsubsection{Local BB-type stepsize}


 


To preserve the distributed property of consensus optimization \eqref{prob:consensus}, we impose a block diagonal structure to the metric. Under any block diagonal metric, the gradient steps are distributable over nodes and the proximal update for consensus set becomes the weighted average over (node-wise) local variables (from Section 3.2). This is highly desirable for large-scale machine learning problems.

Note that, for standard proximal gradient methods, the consensus step is a mere average over local variables. This may not be well suited for most machine learning algorithms where some nodes have larger data subset and thus is likely to be reliable than other nodes. Hence, the updates from such nodes should be given higher weight in the consensus step. Such variable weighing is possible through the (block) diagonal metric selection whereas scalar BB cannot handle.   

% To preserve the distributed property of a variable metric in consensus optimization problems \eqref{prob:consensus}, while optimally utilizing most of the information available in each nodes; we impose a block diagonal structure to the metric. Now (following Section 3.2 \textit{consensus constraint}), the proximal operation for any block diagonal metric in VM-PG can be computed in a distributed fashion. This is highly desirable for large-scale machine learning problems.
% Also note that, for standard proximal gradient methods, the consensus step is a mere averaging operation over local variables in all the nodes. This may not be well suited for most machine learning algorithms where the local loss function is proportional to the data subset size at that particular node. For such cases, the node with the larger data size is likely to provide more information. Hence, an update from such a node should be given higher weight in the consensus step. Such variable weighing is possible through the (block) diagonal metric selection.  
Next we provide two strategies to select the elements of this (block) diagonal metric. The main idea is to approximate the local Hessian $\nabla^2 f_j(x_j^k)$ in each node $j$, only based on the local information, i.e. local step $s_j^k = x_j^k - x_j^{k-1}$ and local gradient change $y_j^k = \nabla f_j(x_j^k) - \nabla f(x_j^{k-1})$. Following this motivation, we propose the below BB - stepsizes, 

%The main idea stems from that the each node approximates its Hessian $\nabla^2 f_j(x_j^k)$ separately, only based on its node (or local) information, i.e., local step $s_j^k = x_j^k - x_j^{k-1}$ and local gradient change $y_j^k = \nabla f_j(x_j^k) - \nabla f(x_j^{k-1})$. This metric selection is well-suited for the observation in the remark above.

\xhdr{Local BB stepsize} Each node evaluates $U_j^k = \alpha_{\mathrm{BB}}(s_j^k, y_j^k)I$ from \eqref{eq:bb_hybrid} based on local $s_j^k $ and $y_j^k$. Then, the metric is given as
\begin{align} \label{eq::localBB}
U^k_{\mathrm{local~BB}} = \text{blkdiag}(U_{1}^k, \ldots, U_{N_{\mathrm{node}}}^k)	.
\end{align}
\xhdr{Local diagonal BB (DBB) stepsize} Similarly, each node evaluates $U_j^k:= U_{\mathrm{DBB}}(s_j^k, y_j^k)$ using \eqref{eq:dbb_solution}. Then, the metric is given as
\begin{align} \label{eq::localDBB}
U^k_{\mathrm{local~DBB}} = \text{blkdiag}(U_{1}^k, \ldots, U_{N_{\mathrm{node}}}^k)	.
\end{align}
Empirical results using the above modifications are provided next.


\subsection{5.2 Experiments}
\xhdr{Consensus $\ell_2^2$ penalized linear/logistic regression}
At each node $j \in \{1,\ldots, N_{\mathrm{node}} \}$, let $a_j^{(i)} \in \reals^n$ and $b_j^{(i)}$ be a sample and its label. Consensus optimization solves
  \begin{align*}
      &\minimize{x} \frac{1}{N} \sum_{j=1}^{N_{\mathrm{node}}} \sum_{i=1}^{N_j} l\left(x_{j};a_j^{(i)}, b_j^{(i)}\right) + \lambda \twonorm{x_j}^2 \\
      &\subjectto x^{j} = z \quad \text{for } \quad j = 1,\ldots, {N_{\mathrm{node}}}
,  \end{align*}
where $N = \sum_{j=1}^{N_{\mathrm{Node}}} N_j$ and $l(x;a,b)$ is a least square or logistic loss . 
  
\xhdr{Synthetic dataset} 
For the consensus optimization problem, we generate synthetic dataset with the size $N$ as in Section 4. In addition, we distribute these dataset over ${N_{\mathrm{node}}}=10$ nodes, i.e., $N = \sum_{j=1}^{N_{\mathrm{node}}} N_j$, so that the size of data subset $N_j$ is proportional to the node number $j$.


\xhdr{VM-PG parameters} For the algorithms, we select $\mu=1.0$ for LS and $\mu=10^{-8}$ for LR respectively. The rest of parameters are kept same as in Section 4. 

\xhdr{Result}
Recall that VM-PG(local BB) and VM-PG (local DBB) method are diagonal metric whose blocks can be different. Fig. \ref{fig:consensus} provide the typical convergence behaviour for all the methods. Here, for most of the cases, VM-PG(local BB) is comparable to or outperforms the PG (BB). In addition, VM-PG (local DBB) provides significant improvement as total sample size $N$ increases. A possible explanation is as the number of samples per-node increases, we get better Hessian approximation in \eqref{eq::localDBB} and hence better convergence results. This shows that VM-PG (local DBB) is very well suited for large-scale machine learning problems. %\sauptik{Additional results are available in supplementary materials}. %In summary, the performance gap between scalar BB stepsize and (diagonal) local-BB type stepsizes gets bigger as the node number $N_{node}$ increase or the size of local data $\mathcal{D}_j$ varies. 

% Recall that PG (global BB) is the standard scalar BB method and VM-PG (global DBB) is diagonal metric where each block $U_j$ is the same over nodes.Recall that VM-PG(local BB) and VM-PG (local DBB) method are diagonal metric whose blocks can be different. Fig. \ref{fig:consensus} provide the typical convergence behaviour for all the methods. Here, VM-PG(local BB) is comparable to or outperforms the PG (BB). Generally, VM-PG (global DBB) and VM-PG (local DBB) converges faster as total sample size increases. For LR with lasso, they eventually outperform PG (global BB) and VM-PG (local DBB) respectively. Additional results are included in the supplementary materials. Overall, the performance gap between global-type methods and local-type methods gets bigger as the node number $N_{node}$ increase or the size of local data $\mathcal{D}_j$ varies. 

% \subsection{Convergence Analysis}\label{sec:convergence}

% Next, we provide the convergence analysis for \eqref{eq:pg_vm}. We begin with some standard assumptions of smoothness and/or (strong) convexity.


% \xhdr{Fixed point iteration}\label{sec:fixed_point} From optimality condition, we can derive the following fixed point algorithm. For a given $U \in \symmpd{n}$, any optimal point $x \in X^F_{opt}$ satisfies %\eqref{cvxopt_composition}
% \begin{align}
%   &0 \in \nabla f(x) + \partial g(x) \label{eq:optimality} \\
%   &\Longleftrightarrow 0 \in x + U^{-1} \partial g(x) - (x - U^{-1} \nabla f(x) ) \nonumber \\
%   % &\Longleftrightarrow   (x - U^{-1} \nabla g(x) ) \in x + U^{-1} \partial h(x)\\
%   &\Longleftrightarrow x = (\Id + U^{-1}  \partial g)^{-1}( \Id - U^{-1} \nabla f) (x) \label{eq:monotone_operator} \\
%   &\Longleftrightarrow x = \prox_{g,U}(x - U^{-1} \nabla f(x) ), \nonumber 
% \end{align}
% where $(\Id + U^{-1}  \partial g)^{-1} (\cdot)$ is called \textit{resolvent operator} and is equivalent to $\prox_{g}^{U}(\cdot)$.\youngsuk{TODO: define subdiff? set...}

% From fixed point theory \cite{parikh2014proximal,rockafellar1976monotone}, it can be demonstrated the proximal gradient method is guaranteed to converge under several sufficient conditions. For examples, it converges linearly when at least one of two operators, $(\Id + U^{-1}  \partial g)^{-1}$ or $( \Id - U^{-1} \nabla f)$, are contractive mapping and the other is non-expansive. By using standard derivation, it can be proved that those sufficient conditions described by the parameters of smoothness and strong convexity of functions can be satisfied for sufficient large metric $U_k$, etc. We include the linear convergence behaviors with proof in the supplementary material for those who are interested in the detailed derivation. 

% \xhdr{Nonmonotone linesearch}\label{sec:linesearch} \youngsuk{TODO}
% However, in many cases it is often difficult to know the (global) parameters such as $L_g$ or $\mu_g$. Moreover, even though such parameters are given, the sufficient condition $\lambda_n \geq L_f/2$ turns out to be too conservative in practice to sufficiently march down toward the optimal point. (\sauptik{did not get the meaning??}). 

% Under this line-search strategy, the algorithm \eqref{algorithm:pg_vm} follows Theorem \eqref{th:convergence}.
% \begin{theorem} \label{th:convergence}
% 	Let $U_k$ is positive definite and bounded above, meaning $0 < \lambda_n < \lambda_1 < \infty$, satisfying \eqref{eq:linesearch}. Then $\lim_{k\rightarrow \infty} F(x^k) := f(x^k) + g(x^k) = F^*$.
% \end{theorem}


% This implies the algorithm \eqref{algorithm:pg_vm} converges linearly ev
% These results implies the followings
% \begin{enumerate}
% 	\item For linear function $g$, i.e., $L =0$, the algorithm converges linearly if $h$ is strongly convex with $\mu_2>0$.
% 	\item Without (strictly)
% \end{enumerate}

